First Observation of $\Lambda\pi^+$ and $\Lambda\pi^-$ Signals near the $\bar{K}N (I=1)$ Mass Threshold in $\Lambda_c^+\rightarrow\Lambda\pi^+\pi^+\pi^-$ Decay

Using the data sample of 980 fb$^{-1}$ collected with the Belle detector operating at the KEKB asymmetric-energy $e^+e^-$ collider, we present the results of an investigation of the $\Lambda\pi^+$ and $\Lambda\pi^-$ invariant mass distributions looking for substructure in the decay $\Lambda_c^+\rightarrow\Lambda\pi^+\pi^+\pi^-$. We find a significant signal in each mass dis\ tribution. When interpreted as resonances, we find for the $\Lambda\pi^+$ ($\Lambda\pi^-$) combination a mass of $1434.3 \pm 0.6 (\mathrm{stat}) \pm 0.9(\mathrm{syst})$ MeV/$c^2$ [$1438.5 \pm 0.9 (\mathrm{stat}) \pm 2.5(\mathrm{syst})$ MeV/$c^2$], an intrinsic width of $11.5 \pm 2.8 (\mathrm{stat}) \pm 5.3(\mathrm{syst})$ MeV/$c^2$ [$33.0 \pm 7.5 (\mathrm{stat}) \pm 23.6(\mathrm{syst})$ MeV/$c^2$] with a significance of 7.5$\sigma$ (6.2$\sigma$). As these two signals are very close to the $\bar{K}N$ threshold, we also investigate the possibility of a $\bar{K}N$ cusp, and find that \ we cannot discriminate between these two interpretations due to the limited size of the data sample.

==> pub631-plain.tex <==
%%% Paper:    Lambda_c+ to Lambda pi pi pi
%%% Journal:  Physical Review Letters
%%% Contacts: Y.Ma, J.Yelton, K.Tanida
%%% Non-responding authors or those who said NO are commented out.
%%% ====================================================================
%%% Click the RELOAD button on your web browser to see the updated file.
%%% ====================================================================
%%% Use \input{author} to insert this material into your latex file.
\noaffiliation
  \author{I.~Adachi} % KEK
% \author{K.~Adamczyk} % Ljubljana
  \author{J.~K.~Ahn} % Korea
  \author{H.~Aihara} % Tokyo
  \author{S.~Al~Said} % Tabuk
  \author{D.~M.~Asner} % BNL
  \author{H.~Atmacan} % Cincinnati
% \author{V.~Aulchenko} % BINP
  \author{T.~Aushev} % HSE
  \author{R.~Ayad} % Tabuk
% \author{T.~Aziz} % Tata
  \author{V.~Babu} % IJCLab
  \author{S.~Bahinipati} % IITB
% \author{A.~M.~Bakich} % Sydney
% \author{Y.~Ban} % Peking
  \author{Sw.~Banerjee} % Louisville
% \author{E.~Barberio} % Melbourne
% \author{M.~Barrett} % KEK
% \author{M.~Bauer} % Karlsruhe
  \author{P.~Behera} % IITM
  \author{K.~Belous} % Protvino
  \author{J.~Bennett} % Mississippi
% \author{F.~Bernlochner} % Bonn
  \author{M.~Bessner} % Hawaii
% \author{D.~Besson} % MEPhI
% \author{V.~Bhardwaj} % IISERM
  \author{B.~Bhuyan} % IITG
  \author{T.~Bilka} % Charles
% \author{S.~Bilokin} % LMU
  \author{D.~Biswas} % Louisville
  \author{A.~Bobrov} % BINP
  \author{D.~Bodrov} % HSE
% \author{A.~Bondar} % BINP
% \author{G.~Bonvicini} % WayneState
  \author{J.~Borah} % IITG
  \author{A.~Bozek} % Krakow
  \author{M.~Bra\v{c}ko} % Ljubljana
  \author{P.~Branchini} % RomaTre
% \author{N.~Braun} % Karlsruhe
  \author{T.~E.~Browder} % Hawaii
  \author{A.~Budano} % RomaTre
  \author{M.~Campajola} % Napoli
% \author{L.~Cao} % DESY
  \author{D.~\v{C}ervenkov} % Charles
  \author{M.-C.~Chang} % FuJen
% \author{P.~Chang} % Taiwan
% \author{V.~Chekelian} % MPI
  \author{A.~Chen} % NCU
% \author{C.~Chen} % ISU
% \author{Y.~Chen} % USTC
% \author{Y.-T.~Chen} % Taiwan
  \author{B.~G.~Cheon} % Hanyang
  \author{K.~Chilikin} % Lebedev
  \author{H.~E.~Cho} % Hanyang
  \author{K.~Cho} % KISTI
  \author{S.-J.~Cho} % Yonsei
  \author{S.-K.~Choi} % CAU
  \author{Y.~Choi} % Sungkyunkwan
  \author{S.~Choudhury} % ISU
  \author{D.~Cinabro} % WayneState
% \author{J.~Cochran} % ISU
% \author{S.~Cunliffe} % DESY
% \author{T.~Czank} % TMU
  \author{S.~Das} % MNIT
% \author{N.~Dash} % IITM
% \author{G.~de~Marino} % IJCLab
  \author{G.~De~Nardo} % Napoli
  \author{G.~De~Pietro} % Karlsruhe
  \author{R.~Dhamija} % IITH
  \author{F.~Di~Capua} % Napoli
  \author{J.~Dingfelder} % Bonn
  \author{Z.~Dole\v{z}al} % Charles
  \author{T.~V.~Dong} % DuyTan
% \author{D.~Dossett} % Melbourne
% \author{S.~Dubey} % Hawaii
% \author{P.~Ecker} % Karlsruhe
  \author{D.~Epifanov} % BINP
% \author{M.~Feindt} % Karlsruhe
  \author{T.~Ferber} % Karlsruhe
  \author{D.~Ferlewicz} % Melbourne
% \author{A.~Frey} % Goettingen
  \author{B.~G.~Fulsom} % PNNL
  \author{R.~Garg} % Panjab
  \author{V.~Gaur} % UPES
% \author{N.~Gabyshev} % BINP
  \author{A.~Garmash} % BINP
  \author{A.~Giri} % IITH
  \author{P.~Goldenzweig} % Karlsruhe
  \author{B.~Golob} % Ljubljana
% \author{G.~Gong} % USTC
  \author{E.~Graziani} % RomaTre
% \author{D.~Greenwald} % TUM
% \author{T.~Gu} % Pittsburgh
% \author{Y.~Guan} % Cincinnati
  \author{K.~Gudkova} % BINP
  \author{C.~Hadjivasiliou} % PNNL
  \author{S.~Halder} % Tata
% \author{X.~Han} % Beihang
% \author{K.~Hara} % KEK
% \author{T.~Hara} % KEK
% \author{O.~Hartbrich} % Hawaii
  \author{K.~Hayasaka} % Niigata
  \author{H.~Hayashii} % Nara
% \author{S.~Hazra} % Tata
  \author{M.~T.~Hedges} % Bonn
% \author{D.~Herrmann} % WayneState
% \author{M.~Hern\'{a}ndez~Villanueva} % DESY
% \author{T.~Higuchi} % IPMU
% \author{S.~Hirose} % Nagoya
  \author{W.-S.~Hou} % Taiwan
  \author{C.-L.~Hsu} % Sydney
% \author{K.~Huang} % Taiwan
% \author{T.~Iijima} % Nagoya
  \author{K.~Inami} % Nagoya
% \author{G.~Inguglia} % Vienna
  \author{N.~Ipsita} % IITH
  \author{A.~Ishikawa} % KEK
  \author{R.~Itoh} % KEK
  \author{M.~Iwasaki} % OsakaCity
% \author{Y.~Iwasaki} % KEK
% \author{S.~Iwata} % TMU
  \author{W.~W.~Jacobs} % Indiana
% \author{I.~Jaegle} % Florida
  \author{E.-J.~Jang} % Gyeongsang
% \author{H.~B.~Jeon} % Kyungpook
% \author{Q.~P.~Ji} % HNU
  \author{S.~Jia} % Fudan
  \author{Y.~Jin} % Trieste
% \author{C.~W.~Joo} % IPMU
% \author{K.~K.~Joo} % Chonnam
% \author{J.~Kahn} % Karlsruhe
% \author{H.~Kakuno} % TMU
% \author{D.~Kalita} % IITG
  \author{A.~B.~Kaliyar} % Vienna
  \author{K.~H.~Kang} % IPMU
% \author{S.~Kang} % ISU
% \author{P.~Kapusta} % Krakow
% \author{G.~Karyan} % DESY
% \author{Y.~Kato} % Nagoya
% \author{H.~Kawai} % Chiba
  \author{T.~Kawasaki} % Kitasato
% \author{H.~Kichimi} % KEK
  \author{C.~Kiesling} % MPI
% \author{B.~H.~Kim} % Seoul
  \author{C.~H.~Kim} % Hanyang
  \author{D.~Y.~Kim} % Soongsil
% \author{H.~J.~Kim} % Kyungpook
% \author{K.-H.~Kim} % KISTI
% \author{K.~T.~Kim} % Korea
% \author{S.~H.~Kim} % Seoul
% \author{S.~K.~Kim} % Seoul
% \author{Y.~J.~Kim} % Korea
  \author{Y.-K.~Kim} % Yonsei
% \author{T.~D.~Kimmel} % VPI
% \author{H.~Kindo} % VPI
  \author{K.~Kinoshita} % Cincinnati
% \author{C.~Kleinwort} % DESY
  \author{P.~Kody\v{s}} % Charles
% \author{I.~Komarov} % DESY
% \author{T.~Konno} % Kitasato
  \author{A.~Korobov} % BINP
  \author{S.~Korpar} % Ljubljana
  \author{E.~Kovalenko} % BINP
  \author{P.~Kri\v{z}an} % Ljubljana
  \author{R.~Kroeger} % Mississippi
% \author{J.-F.~Krohn} % Melbourne
  \author{P.~Krokovny} % BINP
% \author{T.~Kuhr} % LMU
% \author{M.~Kumar} % MNIT
  \author{R.~Kumar} % Punjab
  \author{K.~Kumara} % Mississippi
% \author{T.~Kumita} % TMU
% \author{E.~Kurihara} % Chiba
% \author{A.~Kuzmin} % BINP
% \author{P.~Kvasni\v{c}ka} % Charles
  \author{Y.-J.~Kwon} % Yonsei
% \author{Y.-T.~Lai} % IPMU
% \author{K.~Lalwani} % MNIT
  \author{T.~Lam} % VPI
  \author{J.~S.~Lange} % Giessen
% \author{M.~Laurenza} % RomaTre
% \author{I.~S.~Lee} % Hanyang
% \author{J.~K.~Lee} % Seoul
  \author{S.~C.~Lee} % Kyungpook
% \author{D.~Levit} % KEK
  \author{P.~Lewis} % Bonn
% \author{C.~H.~Li} % LNNU
% \author{J.~Li} % Kyungpook
  \author{L.~K.~Li} % Cincinnati
% \author{S.~X.~Li} % Fudan
  \author{Y.~Li} % Fudan
% \author{Y.~B.~Li} % Fudan
  \author{L.~Li~Gioi} % MPI
  \author{J.~Libby} % IITM
  \author{K.~Lieret} % LMU
  \author{Y.-R.~Lin} % Taiwan
% \author{Z.~Liptak} % Hiroshima
  \author{D.~Liventsev} % WayneState
% \author{A.~Loos} % SouthCarolina
  \author{T.~Luo} % Fudan
  \author{Y.~Ma} % NPC
% \author{J.~MacNaughton} % NPC
% \author{A.~Martini} % DESY
  \author{M.~Masuda} % NPC
  \author{T.~Matsuda} % NPC
  \author{D.~Matvienko} % BINP
  \author{S.~K.~Maurya} % IITG
% \author{J.~T.~McNeil} % Florida
  \author{F.~Meier} % Duke
  \author{M.~Merola} % Napoli
  \author{F.~Metzner} % Bonn
  \author{K.~Miyabayashi} % Nara
% \author{H.~Miyake} % KEK
% \author{H.~Miyata} % Niigata
% \author{R.~Mizuk} % Lebedev
  \author{G.~B.~Mohanty} % Tata
% \author{S.~Mohanty} % Tata
% \author{H.~K.~Moon} % Korea
% \author{T.~J.~Moon} % Seoul
% \author{H.-G.~Moser} % MPI
% \author{M.~Mrvar} % Vienna
% \author{T.~M\"uller} % Karlsruhe
  \author{R.~Mussa} % Torino
  \author{I.~Nakamura} % KEK
% \author{K.~R.~Nakamura} % KEK
% \author{E.~Nakano} % OsakaCity
  \author{T.~Nakano} % NPC
  \author{M.~Nakao} % KEK
% \author{H.~Nakayama} % KEK
% \author{H.~Nakazawa} % Taiwan
% \author{D.~Narwal} % IITG
  \author{Z.~Natkaniec} % Krakow
  \author{A.~Natochii} % Hawaii
  \author{L.~Nayak} % IITH
  \author{M.~Nayak} % TelAviv
% \author{C.~Niebuhr} % DESY
% \author{M.~Niiyama} % NPC
  \author{N.~K.~Nisar} % BNL
  \author{S.~Nishida} % KEK
% \author{K.~Nishimura} % Hawaii
% \author{K.~Ogawa} % Niigata
  \author{S.~Ogawa} % Toho
% \author{S.~Okuno} % Kanagawa
% \author{S.~L.~Olsen} % CAU
  \author{H.~Ono} % NihonDental
% \author{Y.~Onuki} % Tokyo
  \author{P.~Oskin} % Lebedev
% \author{H.~Ozaki} % KEK
  \author{P.~Pakhlov} % Lebedev
  \author{G.~Pakhlova} % HSE
% \author{T.~Pang} % Pittsburgh
  \author{S.~Pardi} % Napoli
  \author{H.~Park} % Kyungpook
  \author{J.~Park} % Yonsei
% \author{S.-H.~Park} % KEK
% \author{A.~Passeri} % RomaTre
  \author{S.~Patra} % IISERM
  \author{S.~Paul} % TUM
% \author{T.~K.~Pedlar} % Luther
  \author{R.~Pestotnik} % Ljubljana
% \author{F.~Pham} % Melbourne
  \author{L.~E.~Piilonen} % VPI
  \author{T.~Podobnik} % Ljubljana
% \author{V.~Popov} % HSE
% \author{S.~Prell} % ISU
  \author{E.~Prencipe} % Giessen
  \author{M.~T.~Prim} % Bonn
% \author{M.~V.~Purohit} % OIST
% \author{A.~Rabusov} % TUM
% \author{P.~K.~Resmi} % IITM
% \author{M.~Ritter} % LMU
% \author{M.~R\"{o}hrken} % DESY
  \author{A.~Rostomyan} % DESY
  \author{N.~Rout} % IITM
% \author{M.~Rozanska} % Krakow
  \author{G.~Russo} % Napoli
% \author{D.~Sahoo} % ISU
% \author{Y.~Sakai} % KEK
% \author{M.~Salehi} % Malaya
  \author{S.~Sandilya} % IITH
% \author{A.~Sangal} % Cincinnati
  \author{L.~Santelj} % Ljubljana
% \author{T.~Sanuki} % Tohoku
% \author{Y.~Sato} % KEK
  \author{V.~Savinov} % Pittsburgh
% \author{P.~Schmolz} % LMU
% \author{O.~Schneider} % Lausanne
  \author{G.~Schnell} % Bilbao
  \author{J.~Schueler} % Hawaii
  \author{C.~Schwanda} % Vienna
% \author{A.~J.~Schwartz} % Cincinnati
% \author{B.~Schwenker} % Goettingen
% \author{R.~Seidl} % RIKEN
  \author{Y.~Seino} % Niigata
  \author{K.~Senyo} % Yamagata
% \author{O.~Seon} % Nagoya
% \author{I.~S.~Seong} % Hawaii
  \author{M.~E.~Sevior} % Melbourne
  \author{W.~Shan} % HUNNU
  \author{M.~Shapkin} % Protvino
  \author{C.~Sharma} % MNIT
% \author{V.~Shebalin} % Hawaii
  \author{C.~P.~Shen} % Fudan
% \author{H.~Shibuya} % Toho
  \author{J.-G.~Shiu} % Taiwan
% \author{B.~Shwartz} % BINP
% \author{A.~Sibidanov} % Hawaii
  \author{F.~Simon} % MPI
% \author{J.~B.~Singh} % Panjab
% \author{R.~Sinha} % IMSC
% \author{K.~Smith} % Melbourne
  \author{A.~Sokolov} % Protvino
% \author{Y.~Soloviev} % DESY
  \author{E.~Solovieva} % Lebedev
% \author{S.~Stani\v{c}} % NovaGorica
  \author{M.~Stari\v{c}} % Ljubljana
% \author{Z.~S.~Stottler} % VPI
% \author{J.~F.~Strube} % PNNL
% \author{J.~Stypula} % Krakow
  \author{M.~Sumihama} % NPC
% \author{K.~Sumisawa} % KEK
  \author{T.~Sumiyoshi} % TMU
  \author{W.~Sutcliffe} % Bonn
% \author{S.~Y.~Suzuki} % KEK
  \author{M.~Takizawa} % NPC
  \author{U.~Tamponi} % Torino
% \author{S.~Tanaka} % KEK
% \author{S.~S.~Tang} % Fudan
  \author{K.~Tanida} % NPC
% \author{N.~Taniguchi} % KEK
% \author{Y.~Tao} % Florida
% \author{G.~N.~Taylor} % Melbourne
  \author{F.~Tenchini} % Pisa
% \author{Y.~Teramoto} % OsakaCity
% \author{A.~Thampi} % Juelich
% \author{R.~Tiwary} % Tata
% \author{K.~Trabelsi} % IJCLab
% \author{T.~Tsuboyama} % KEK
  \author{M.~Uchida} % NPC
% \author{I.~Ueda} % KEK
  \author{S.~Uehara} % KEK
  \author{T.~Uglov} % Lebedev
  \author{Y.~Unno} % Hanyang
  \author{K.~Uno} % Niigata
  \author{S.~Uno} % KEK
  \author{P.~Urquijo} % Melbourne
% \author{Y.~Ushiroda} % KEK
  \author{Y.~Usov} % BINP
  \author{S.~E.~Vahsen} % Hawaii
  \author{R.~Van~Tonder} % Bonn
  \author{G.~Varner} % Hawaii
% \author{K.~E.~Varvell} % Sydney
  \author{A.~Vinokurova} % BINP
% \author{V.~Vorobyev} % BINP
  \author{A.~Vossen} % Duke
% \author{E.~Waheed} % KEK
% \author{B.~Wang} % MPI
% \author{C.~H.~Wang} % NUU
  \author{D.~Wang} % Florida
% \author{E.~Wang} % Pittsburgh
  \author{M.-Z.~Wang} % Taiwan
% \author{X.~L.~Wang} % Fudan
  \author{M.~Watanabe} % Niigata
% \author{Y.~Watanabe} % Kanagawa
  \author{S.~Watanuki} % Yonsei
% \author{S.~Wehle} % DESY
  \author{O.~Werbycka} % Trieste
% \author{E.~Widmann} % Vienna
% \author{J.~Wiechczynski} % Krakow
  \author{E.~Won} % Korea
  \author{X.~Xu} % Soochow
  \author{B.~D.~Yabsley} % Sydney
% \author{S.~Yamada} % KEK
% \author{H.~Yamamoto} % Tohoku
  \author{W.~Yan} % USTC
  \author{S.~B.~Yang} % Korea
% \author{H.~Ye} % DESY
  \author{J.~Yelton} % Florida
  \author{J.~H.~Yin} % Korea
% \author{Y.~Yook} % IHEP
  \author{C.~Z.~Yuan} % IHEP
  \author{L.~Yuan} % Beihang
% \author{Y.~Yusa} % Niigata
% \author{Y.~Zhai} % ISU
% \author{J.~Zhang} % IHEP
  \author{Z.~P.~Zhang} % USTC
  \author{V.~Zhilich} % BINP
  \author{V.~Zhukova} % Lebedev
% \author{V.~Zhulanov} % BINP
\collaboration{The Belle Collaboration}


==> pub631.tex <==
%%% Paper:    Lambda_c+ to Lambda pi pi pi
%%% Journal:  Physical Review Letters
%%% Contacts: Y.Ma, J.Yelton, K.Tanida
%%% Non-responding authors or those who said NO are commented out.
%%% ====================================================================
%%% Click the RELOAD button on your web browser to see the updated file.
%%% ====================================================================
%%% Use \input{author} to insert this material into your latex file.
%%%%% Force institutions to appear in alphabetical order when typeset.
\noaffiliation
\newcommand{\instGoettingen}{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"{o}ttingen, 37073 G\"{o}ttingen}
\newcommand{\instBeihang}{Beihang University, Beijing 100191}
\newcommand{\instBNL}{Brookhaven National Laboratory, Upton, New York 11973}
\newcommand{\instBINP}{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}
\newcommand{\instCMU}{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213}
\newcommand{\instPrague}{Faculty of Mathematics and Physics, Charles University, 121 16 Prague}
\newcommand{\instChiba}{Chiba University, Chiba 263-8522}
\newcommand{\instChonnam}{Chonnam National University, Gwangju 61186}
\newcommand{\instCAU}{Chung-Ang University, Seoul 06974}
\newcommand{\instDESY}{Deutsches Elektronen--Synchrotron, 22607 Hamburg}
\newcommand{\instDuke}{Duke University, Durham, North Carolina 27708}
\newcommand{\instITAR}{Institute of Theoretical and Applied Research (ITAR), Duy Tan University, Hanoi 100000}
\newcommand{\instEPFL}{\'Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Lausanne 1015}
\newcommand{\instJuelich}{Forschungszentrum J\"{u}lich, 52425 J\"{u}lich}
\newcommand{\instFuJen}{Department of Physics, Fu Jen Catholic University, Taipei 24205}
\newcommand{\instFudan}{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443}
\newcommand{\instGifu}{Gifu University, Gifu 501-1193}
\newcommand{\instSOKENDAI}{The Graduate University for Advanced Studies (Sokendai), Tsukuba 305-0801}
\newcommand{\instGyeongsang}{Gyeongsang National University, Jinju 52828}
\newcommand{\instHanyang}{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763}
\newcommand{\instHNU}{Henan Normal University, Xinxiang 453007}
\newcommand{\instKEK}{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}
\newcommand{\instJPARC}{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}
\newcommand{\instHiroshima}{Hiroshima University, Higashi-Hiroshima, Hiroshima 739-8530}
\newcommand{\instHUNNU}{Hunan Normal University, Changsha 410081}
\newcommand{\instIKERBASQUE}{IKERBASQUE, Basque Foundation for Science, 48013 Bilbao}
\newcommand{\instNapoliINFN}{INFN Sezione di Napoli, I-80126 Napoli}
\newcommand{\instPisaINFN}{INFN Sezione di Pisa, I-56127 Pisa}
\newcommand{\instRomaTreINFN}{INFN Sezione di Roma Tre, I-00146 Roma}
\newcommand{\instTorinoINFN}{INFN Sezione di Torino, I-10125 Torino}
\newcommand{\instTriesteINFN}{INFN Sezione di Trieste, I-34127 Trieste}
\newcommand{\instIISER}{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306}
\newcommand{\instIITBhubaneswar}{Indian Institute of Technology Bhubaneswar, Bhubaneswar 752050}
\newcommand{\instIITGuwahati}{Indian Institute of Technology Guwahati, Assam 781039}
\newcommand{\instIITHyderabad}{Indian Institute of Technology Hyderabad, Telangana 502285}
\newcommand{\instIITMadras}{Indian Institute of Technology Madras, Chennai 600036}
\newcommand{\instIndiana}{Indiana University, Bloomington, Indiana 47408}
\newcommand{\instIHEPRussia}{Institute for High Energy Physics, Protvino 142281}
\newcommand{\instHEPHYVienna}{Institute of High Energy Physics, Vienna 1050}
\newcommand{\instIHEPChina}{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049}
\newcommand{\instChennai}{Institute of Mathematical Sciences, Chennai 600113}
\newcommand{\instISU}{Iowa State University, Ames, Iowa 50011}
\newcommand{\instJAEA}{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195}
\newcommand{\instKanagawa}{Kanagawa University, Yokohama 221-8686}
\newcommand{\instKarlsruhe}{Institut f\"{u}r Experimentelle Teilchenphysik, Karlsruher Institut f\"{u}r Technologie, 76131 Karlsruhe}
\newcommand{\instKAU}{Department of Physics, Faculty of Science, King Abdulaziz University, Jeddah 21589}
\newcommand{\instKitasato}{Kitasato University, Sagamihara 252-0373}
\newcommand{\instKISTI}{Korea Institute of Science and Technology Information, Daejeon 34141}
\newcommand{\instKoreaUnivKU}{Korea University, Seoul 02841}
\newcommand{\instKSU}{Kyoto Sangyo University, Kyoto 603-8555}
\newcommand{\instKyungpook}{Kyungpook National University, Daegu 41566}
\newcommand{\instLNNU}{Liaoning Normal University, Dalian 116029}
\newcommand{\instGiessen}{Justus-Liebig-Universit\"{a}t Gie\ss{}en, 35392 Gie\ss{}en}
\newcommand{\instLuther}{Luther College, Decorah, Iowa 52101}
\newcommand{\instMNITJaipur}{Malaviya National Institute of Technology Jaipur, Jaipur 302017}
\newcommand{\instLMU}{Ludwig Maximilians University, 80539 Munich}
\newcommand{\instSMI}{Stefan Meyer Institute for Subatomic Physics, Vienna 1090}
\newcommand{\instMEPhI}{Moscow Physical Engineering Institute, Moscow 115409}
\newcommand{\instNagoya}{Graduate School of Science, Nagoya University, Nagoya 464-8602}
\newcommand{\instNagoyaKMI}{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602}
\newcommand{\instNaraWu}{Nara Women's University, Nara 630-8506}
\newcommand{\instNCU}{National Central University, Chung-li 32054}
\newcommand{\instHSE}{National Research University Higher School of Economics, Moscow 101000}
\newcommand{\instNTUTaiwan}{Department of Physics, National Taiwan University, Taipei 10617}
\newcommand{\instNUUTaiwan}{National United University, Miao Li 36003}
\newcommand{\instKrakow}{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342}
\newcommand{\instNiigata}{Niigata University, Niigata 950-2181}
\newcommand{\instNDU}{Nippon Dental University, Niigata 951-8580}
\newcommand{\instNSU}{Novosibirsk State University, Novosibirsk 630090}
\newcommand{\instOkinawa}{Okinawa Institute of Science and Technology, Okinawa 904-0495}
\newcommand{\instOsakaMetropolitan}{Osaka Metropolitan University, Osaka 558-8585}
\newcommand{\instRCNP}{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047}
\newcommand{\instPNNL}{Pacific Northwest National Laboratory, Richland, Washington 99352}
\newcommand{\instPanjab}{Panjab University, Chandigarh 160014}
\newcommand{\instPeking}{Peking University, Beijing 100871}
\newcommand{\instMPP}{Max-Planck-Institut f\"{u}r Physik, 80805 M\"{u}nchen}
\newcommand{\instPanjabPAU}{Punjab Agricultural University, Ludhiana 141004}
\newcommand{\instRIKENMSL}{Meson Science Laboratory, Cluster for Pioneering Research, RIKEN, Saitama 351-0198}
\newcommand{\instRIKENBNL}{RIKEN BNL Research Center, Upton, New York 11973}
\newcommand{\instSeoul}{Seoul National University, Seoul 08826}
\newcommand{\instSPU}{Showa Pharmaceutical University, Tokyo 194-8543}
\newcommand{\instSoochow}{Soochow University, Suzhou 215006}
\newcommand{\instSoongsil}{Department of Physics and Origin of Matter and Evolution of Galaxy (OMEG) Institute, Soongsil University, Seoul 06978}
\newcommand{\instLjubljanaJSI}{J. Stefan Institute, 1000 Ljubljana}
\newcommand{\instSKKU}{Sungkyunkwan University, Suwon 16419}
\newcommand{\instTata}{Tata Institute of Fundamental Research, Mumbai 400005}
\newcommand{\instTUM}{Department of Physics, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching}
\newcommand{\instTelAviv}{School of Physics and Astronomy, Tel Aviv University, Tel Aviv 69978}
\newcommand{\instToho}{Toho University, Funabashi 274-8510}
\newcommand{\instTohoku}{Department of Physics, Tohoku University, Sendai 980-8578}
\newcommand{\instTitech}{Tokyo Institute of Technology, Tokyo 152-8550}
\newcommand{\instTokyoMetropolitan}{Tokyo Metropolitan University, Tokyo 192-0397}
\newcommand{\instNapoliUNIV}{Dipartimento di Scienze Fisiche, Universit\`{a} di Napoli Federico II, I-80126 Napoli}
\newcommand{\instPisaUNIV}{Dipartimento di Fisica, Universit\`{a} di Pisa, I-56127 Pisa}
\newcommand{\instRomaTreUNIV}{Dipartimento di Matematica e Fisica, Universit\`{a} di Roma Tre, I-00146 Roma}
\newcommand{\instIJCLab}{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay}
\newcommand{\instBilbao}{Department of Physics \& EHU Quantum Center, University of the Basque Country UPV/EHU, 48080 Bilbao}
\newcommand{\instBonn}{University of Bonn, 53115 Bonn}
\newcommand{\instCincinnati}{University of Cincinnati, Cincinnati, Ohio 45221}
\newcommand{\instFlorida}{University of Florida, Gainesville, Florida 32611}
\newcommand{\instHawaii}{University of Hawaii, Honolulu, Hawaii 96822}
\newcommand{\instLjubljanaUniLJ}{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana}
\newcommand{\instLouisville}{University of Louisville, Louisville, Kentucky 40292}
\newcommand{\instMalaya}{National Centre for Particle Physics, University of Malaya, 50603 Kuala Lumpur}
\newcommand{\instLjubljanaUM}{Faculty of Chemistry and Chemical Engineering, University of Maribor, 2000 Maribor}
\newcommand{\instMelbourne}{School of Physics, University of Melbourne, Victoria 3010}
\newcommand{\instMississippi}{University of Mississippi, University, Mississippi 38677}
\newcommand{\instUOM}{University of Miyazaki, Miyazaki 889-2192}
\newcommand{\instNovaGorica}{University of Nova Gorica, 5000 Nova Gorica}
\newcommand{\instUPES}{University of Petroleum and Energy Studies, Dehradun 248007}
\newcommand{\instPittsburgh}{University of Pittsburgh, Pittsburgh, Pennsylvania 15260}
\newcommand{\instUSTC}{Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei 230026}
\newcommand{\instSydney}{School of Physics, University of Sydney, New South Wales 2006}
\newcommand{\instTabuk}{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451}
\newcommand{\instUTokyo}{Department of Physics, University of Tokyo, Tokyo 113-0033}
\newcommand{\instEri}{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032}
\newcommand{\instIPMU}{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583}
\newcommand{\instUtkal}{Utkal University, Bhubaneswar 751004}
\newcommand{\instVPI}{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061}
\newcommand{\instWayneState}{Wayne State University, Detroit, Michigan 48202}
\newcommand{\instYamagata}{Yamagata University, Yamagata 990-8560}
\newcommand{\instYonsei}{Yonsei University, Seoul 03722}
%%%\affiliation{\instGoettingen}
\affiliation{\instBeihang}
\affiliation{\instBNL}
\affiliation{\instBINP}
\affiliation{\instCMU}
\affiliation{\instPrague}
%%%\affiliation{\instChiba}
%%%\affiliation{\instChonnam}
\affiliation{\instCAU}
\affiliation{\instDESY}
\affiliation{\instDuke}
\affiliation{\instITAR}
%%%\affiliation{\instEPFL}
%%%\affiliation{\instJuelich}
\affiliation{\instFuJen}
\affiliation{\instFudan}
\affiliation{\instGifu}
\affiliation{\instSOKENDAI}
\affiliation{\instGyeongsang}
\affiliation{\instHanyang}
%%%\affiliation{\instHNU}
\affiliation{\instKEK}
\affiliation{\instJPARC}
%%%\affiliation{\instHiroshima}
\affiliation{\instHUNNU}
\affiliation{\instIKERBASQUE}
\affiliation{\instNapoliINFN}
\affiliation{\instPisaINFN}
\affiliation{\instRomaTreINFN}
\affiliation{\instTorinoINFN}
\affiliation{\instTriesteINFN}
\affiliation{\instIISER}
\affiliation{\instIITBhubaneswar}
\affiliation{\instIITGuwahati}
\affiliation{\instIITHyderabad}
\affiliation{\instIITMadras}
\affiliation{\instIndiana}
\affiliation{\instIHEPRussia}
\affiliation{\instHEPHYVienna}
\affiliation{\instIHEPChina}
%%%\affiliation{\instChennai}
\affiliation{\instISU}
\affiliation{\instJAEA}
%%%\affiliation{\instKanagawa}
\affiliation{\instKarlsruhe}
\affiliation{\instKAU}
\affiliation{\instKitasato}
\affiliation{\instKISTI}
\affiliation{\instKoreaUnivKU}
%%%\affiliation{\instKSU}
\affiliation{\instKyungpook}
%%%\affiliation{\instLNNU}
\affiliation{\instGiessen}
%%%\affiliation{\instLuther}
\affiliation{\instMNITJaipur}
\affiliation{\instLMU}
%%%\affiliation{\instSMI}
%%%\affiliation{\instMEPhI}
\affiliation{\instNagoya}
%%%\affiliation{\instNagoyaKMI}
\affiliation{\instNaraWu}
\affiliation{\instNCU}
\affiliation{\instHSE}
\affiliation{\instNTUTaiwan}
%%%\affiliation{\instNUUTaiwan}
\affiliation{\instKrakow}
\affiliation{\instNiigata}
\affiliation{\instNDU}
\affiliation{\instNSU}
%%%\affiliation{\instOkinawa}
\affiliation{\instOsakaMetropolitan}
\affiliation{\instRCNP}
\affiliation{\instPNNL}
\affiliation{\instPanjab}
%%%\affiliation{\instPeking}
\affiliation{\instMPP}
\affiliation{\instPanjabPAU}
\affiliation{\instRIKENMSL}
%%%\affiliation{\instRIKENBNL}
%%%\affiliation{\instSeoul}
\affiliation{\instSPU}
\affiliation{\instSoochow}
\affiliation{\instSoongsil}
\affiliation{\instLjubljanaJSI}
\affiliation{\instSKKU}
\affiliation{\instTata}
\affiliation{\instTUM}
\affiliation{\instTelAviv}
\affiliation{\instToho}
%%%\affiliation{\instTohoku}
\affiliation{\instTitech}
\affiliation{\instTokyoMetropolitan}
\affiliation{\instNapoliUNIV}
\affiliation{\instPisaUNIV}
%%%\affiliation{\instRomaTreUNIV}
\affiliation{\instIJCLab}
\affiliation{\instBilbao}
\affiliation{\instBonn}
\affiliation{\instCincinnati}
\affiliation{\instFlorida}
\affiliation{\instHawaii}
\affiliation{\instLjubljanaUniLJ}
\affiliation{\instLouisville}
%%%\affiliation{\instMalaya}
\affiliation{\instLjubljanaUM}
\affiliation{\instMelbourne}
\affiliation{\instMississippi}
\affiliation{\instUOM}
%%%\affiliation{\instNovaGorica}
\affiliation{\instUPES}
\affiliation{\instPittsburgh}
\affiliation{\instUSTC}
\affiliation{\instSydney}
\affiliation{\instTabuk}
\affiliation{\instUTokyo}
\affiliation{\instEri}
\affiliation{\instIPMU}
%%%\affiliation{\instUtkal}
\affiliation{\instVPI}
\affiliation{\instWayneState}
\affiliation{\instYamagata}
\affiliation{\instYonsei}
  \author{Y.~Ma}\affiliation{\instRIKENMSL} % NPC
  \author{J.~Yelton}\affiliation{\instFlorida} % Florida
  \author{K.~Tanida}\affiliation{\instJAEA} % NPC
  \author{I.~Adachi}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{K.~Adamczyk}\affiliation{\instLjubljanaJSI} % Ljubljana
  \author{J.~K.~Ahn}\affiliation{\instKoreaUnivKU} % Korea
  \author{H.~Aihara}\affiliation{\instUTokyo} % Tokyo
  \author{S.~Al~Said}\affiliation{\instTabuk}\affiliation{\instKAU} % Tabuk
  \author{D.~M.~Asner}\affiliation{\instBNL} % BNL
  \author{H.~Atmacan}\affiliation{\instCincinnati} % Cincinnati
% \author{V.~Aulchenko}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{T.~Aushev}\affiliation{\instHSE} % HSE
  \author{R.~Ayad}\affiliation{\instTabuk} % Tabuk
% \author{T.~Aziz}\affiliation{\instTata} % Tata
  \author{V.~Babu}\affiliation{\instIJCLab} % IJCLab
  \author{S.~Bahinipati}\affiliation{\instIITBhubaneswar} % IITB
% \author{A.~M.~Bakich}\affiliation{\instSydney} % Sydney
% \author{Y.~Ban}\affiliation{\instPeking} % Peking
  \author{Sw.~Banerjee}\affiliation{\instLouisville} % Louisville
% \author{E.~Barberio}\affiliation{\instMelbourne} % Melbourne
% \author{M.~Barrett}\affiliation{\instKEK} % KEK
% \author{M.~Bauer}\affiliation{\instKarlsruhe} % Karlsruhe
  \author{P.~Behera}\affiliation{\instIITMadras} % IITM
  \author{K.~Belous}\affiliation{\instIHEPRussia} % Protvino
  \author{J.~Bennett}\affiliation{\instMississippi} % Mississippi
% \author{F.~Bernlochner}\affiliation{\instBonn} % Bonn
  \author{M.~Bessner}\affiliation{\instHawaii} % Hawaii
% \author{D.~Besson}\affiliation{\instMEPhI} % MEPhI
% \author{V.~Bhardwaj}\affiliation{\instIISER} % IISERM
  \author{B.~Bhuyan}\affiliation{\instIITGuwahati} % IITG
  \author{T.~Bilka}\affiliation{\instPrague} % Charles
% \author{S.~Bilokin}\affiliation{\instLMU} % LMU
  \author{D.~Biswas}\affiliation{\instLouisville} % Louisville
  \author{A.~Bobrov}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{D.~Bodrov}\affiliation{\instHSE} % HSE
% \author{A.~Bondar}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
% \author{G.~Bonvicini}\affiliation{\instWayneState} % WayneState
  \author{J.~Borah}\affiliation{\instIITGuwahati} % IITG
  \author{A.~Bozek}\affiliation{\instKrakow} % Krakow
  \author{M.~Bra\v{c}ko}\affiliation{\instLjubljanaUM}\affiliation{\instLjubljanaJSI} % Ljubljana
  \author{P.~Branchini}\affiliation{\instRomaTreINFN} % RomaTre
  \author{T.~E.~Browder}\affiliation{\instHawaii} % Hawaii
  \author{A.~Budano}\affiliation{\instRomaTreINFN} % RomaTre
  \author{M.~Campajola}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % Napoli
% \author{L.~Cao}\affiliation{\instDESY} % DESY
  \author{D.~\v{C}ervenkov}\affiliation{\instPrague} % Charles
  \author{M.-C.~Chang}\affiliation{\instFuJen} % FuJen
% \author{P.~Chang}\affiliation{\instNTUTaiwan} % Taiwan
% \author{V.~Chekelian}\affiliation{\instMPP} % MPI
  \author{A.~Chen}\affiliation{\instNCU} % NCU
% \author{C.~Chen}\affiliation{\instISU} % ISU
% \author{Y.~Chen}\affiliation{\instUSTC} % USTC
% \author{Y.-T.~Chen}\affiliation{\instNTUTaiwan} % Taiwan
  \author{B.~G.~Cheon}\affiliation{\instHanyang} % Hanyang
  \author{K.~Chilikin}\affiliation{\instBINP} % BINP
  \author{H.~E.~Cho}\affiliation{\instHanyang} % Hanyang
  \author{K.~Cho}\affiliation{\instKISTI} % KISTI
  \author{S.-J.~Cho}\affiliation{\instYonsei} % Yonsei
  \author{S.-K.~Choi}\affiliation{\instCAU} % CAU
  \author{Y.~Choi}\affiliation{\instSKKU} % Sungkyunkwan
  \author{S.~Choudhury}\affiliation{\instISU} % ISU
  \author{D.~Cinabro}\affiliation{\instWayneState} % WayneState
% \author{J.~Cochran}\affiliation{\instISU} % ISU
% \author{S.~Cunliffe}\affiliation{\instDESY} % DESY
% \author{T.~Czank}\affiliation{\instTokyoMetropolitan} % TMU
  \author{S.~Das}\affiliation{\instMNITJaipur} % MNIT
% \author{N.~Dash}\affiliation{\instIITMadras} % IITM
% \author{G.~de~Marino}\affiliation{\instIJCLab} % IJCLab
  \author{G.~De~Nardo}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % Napoli
  \author{G.~De~Pietro}\affiliation{\instKarlsruhe} % Karlsruhe
  \author{R.~Dhamija}\affiliation{\instIITHyderabad} % IITH
  \author{F.~Di~Capua}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % Napoli
  \author{J.~Dingfelder}\affiliation{\instBonn} % Bonn
  \author{Z.~Dole\v{z}al}\affiliation{\instPrague} % Charles
  \author{T.~V.~Dong}\affiliation{\instITAR} % DuyTan
% \author{D.~Dossett}\affiliation{\instMelbourne} % Melbourne
% \author{S.~Dubey}\affiliation{\instHawaii} % Hawaii
% \author{P.~Ecker}\affiliation{\instKarlsruhe} % Karlsruhe
  \author{D.~Epifanov}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
% \author{M.~Feindt}\affiliation{\instKarlsruhe} % Karlsruhe
  \author{T.~Ferber}\affiliation{\instKarlsruhe} % Karlsruhe
  \author{D.~Ferlewicz}\affiliation{\instMelbourne} % Melbourne
% \author{A.~Frey}\affiliation{\instGoettingen} % Goettingen
  \author{B.~G.~Fulsom}\affiliation{\instPNNL} % PNNL
  \author{R.~Garg}\affiliation{\instCMU} % CMU
  \author{V.~Gaur}\affiliation{\instUPES} % UPES
% \author{N.~Gabyshev}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{A.~Garmash}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{A.~Giri}\affiliation{\instIITHyderabad} % IITH
  \author{P.~Goldenzweig}\affiliation{\instKarlsruhe} % Karlsruhe
  \author{B.~Golob}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{G.~Gong}\affiliation{\instUSTC} % USTC
  \author{E.~Graziani}\affiliation{\instRomaTreINFN} % RomaTre
% \author{D.~Greenwald}\affiliation{\instTUM} % TUM
% \author{T.~Gu}\affiliation{\instPittsburgh} % Pittsburgh
% \author{Y.~Guan}\affiliation{\instCincinnati} % Cincinnati
  \author{K.~Gudkova}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{C.~Hadjivasiliou}\affiliation{\instPNNL} % PNNL
  \author{S.~Halder}\affiliation{\instTata} % Tata
% \author{X.~Han}\affiliation{\instBeihang} % Beihang
% \author{K.~Hara}\affiliation{\instKEK} % KEK
% \author{T.~Hara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{O.~Hartbrich}\affiliation{\instHawaii} % Hawaii
  \author{K.~Hayasaka}\affiliation{\instNiigata} % Niigata
  \author{H.~Hayashii}\affiliation{\instNaraWu} % Nara
% \author{S.~Hazra}\affiliation{\instTata} % Tata
  \author{M.~T.~Hedges}\affiliation{\instBonn} % Bonn
% \author{D.~Herrmann}\affiliation{\instWayneState} % WayneState
% \author{M.~Hern\'{a}ndez~Villanueva}\affiliation{\instDESY} % DESY
% \author{T.~Higuchi}\affiliation{\instIPMU} % IPMU
  \author{W.-S.~Hou}\affiliation{\instNTUTaiwan} % Taiwan
  \author{C.-L.~Hsu}\affiliation{\instSydney} % Sydney
% \author{K.~Huang}\affiliation{\instNTUTaiwan} % Taiwan
% \author{T.~Iijima}\affiliation{\instNagoyaKMI}\affiliation{\instNagoya} % Nagoya
  \author{K.~Inami}\affiliation{\instNagoya} % Nagoya
% \author{G.~Inguglia}\affiliation{\instHEPHYVienna} % Vienna
  \author{N.~Ipsita}\affiliation{\instIITHyderabad} % IITH
  \author{A.~Ishikawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
  \author{R.~Itoh}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
  \author{M.~Iwasaki}\affiliation{\instOsakaMetropolitan} % OsakaCity
% \author{Y.~Iwasaki}\affiliation{\instKEK} % KEK
% \author{S.~Iwata}\affiliation{\instTokyoMetropolitan} % TMU
  \author{W.~W.~Jacobs}\affiliation{\instIndiana} % Indiana
  \author{E.-J.~Jang}\affiliation{\instGyeongsang} % Gyeongsang
% \author{H.~B.~Jeon}\affiliation{\instKyungpook} % Kyungpook
% \author{Q.~P.~Ji}\affiliation{\instHNU} % HNU
  \author{S.~Jia}\affiliation{\instFudan} % Fudan
  \author{Y.~Jin}\affiliation{\instTriesteINFN} % Trieste
% \author{K.~K.~Joo}\affiliation{\instChonnam} % Chonnam
% \author{J.~Kahn}\affiliation{\instKarlsruhe} % Karlsruhe
% \author{H.~Kakuno}\affiliation{\instTokyoMetropolitan} % TMU
% \author{D.~Kalita}\affiliation{\instIITGuwahati} % IITG
  \author{A.~B.~Kaliyar}\affiliation{\instHEPHYVienna} % Vienna
  \author{K.~H.~Kang}\affiliation{\instIPMU} % IPMU
% \author{S.~Kang}\affiliation{\instISU} % ISU
% \author{P.~Kapusta}\affiliation{\instKrakow} % Krakow
% \author{G.~Karyan}\affiliation{\instDESY} % DESY
% \author{Y.~Kato}\affiliation{\instNagoya} % Nagoya
% \author{H.~Kawai}\affiliation{\instChiba} % Chiba
  \author{T.~Kawasaki}\affiliation{\instKitasato} % Kitasato
% \author{H.~Kichimi}\affiliation{\instKEK} % KEK
  \author{C.~Kiesling}\affiliation{\instMPP} % MPI
  \author{C.~H.~Kim}\affiliation{\instHanyang} % Hanyang
  \author{D.~Y.~Kim}\affiliation{\instSoongsil} % Soongsil
% \author{H.~J.~Kim}\affiliation{\instKyungpook} % Kyungpook
% \author{K.-H.~Kim}\affiliation{\instKISTI} % KISTI
% \author{K.~T.~Kim}\affiliation{\instKoreaUnivKU} % Korea
% \author{S.~K.~Kim}\affiliation{\instSeoul} % Seoul
% \author{Y.~J.~Kim}\affiliation{\instKoreaUnivKU} % Korea
  \author{Y.-K.~Kim}\affiliation{\instYonsei} % Yonsei
% \author{T.~D.~Kimmel}\affiliation{\instVPI} % VPI
% \author{H.~Kindo}\affiliation{\instVPI}\affiliation{\instKEK} % VPI
  \author{K.~Kinoshita}\affiliation{\instCincinnati} % Cincinnati
% \author{C.~Kleinwort}\affiliation{\instDESY} % DESY
  \author{P.~Kody\v{s}}\affiliation{\instPrague} % Charles
% \author{I.~Komarov}\affiliation{\instDESY} % DESY
% \author{T.~Konno}\affiliation{\instKitasato} % Kitasato
  \author{A.~Korobov}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{S.~Korpar}\affiliation{\instLjubljanaUM}\affiliation{\instLjubljanaJSI} % Ljubljana
  \author{E.~Kovalenko}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{P.~Kri\v{z}an}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{R.~Kroeger}\affiliation{\instMississippi} % Mississippi
% \author{J.-F.~Krohn}\affiliation{\instMelbourne} % Melbourne
  \author{P.~Krokovny}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
% \author{T.~Kuhr}\affiliation{\instLMU} % LMU
% \author{M.~Kumar}\affiliation{\instMNITJaipur} % MNIT
  \author{R.~Kumar}\affiliation{\instPanjabPAU} % Punjab
  \author{K.~Kumara}\affiliation{\instMississippi} % Mississippi
% \author{T.~Kumita}\affiliation{\instTokyoMetropolitan} % TMU
% \author{E.~Kurihara}\affiliation{\instChiba} % Chiba
% \author{A.~Kuzmin}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
% \author{P.~Kvasni\v{c}ka}\affiliation{\instPrague} % Charles
  \author{Y.-J.~Kwon}\affiliation{\instYonsei} % Yonsei
% \author{Y.-T.~Lai}\affiliation{\instIPMU} % IPMU
% \author{K.~Lalwani}\affiliation{\instMNITJaipur} % MNIT
  \author{T.~Lam}\affiliation{\instVPI} % VPI
  \author{J.~S.~Lange}\affiliation{\instGiessen} % Giessen
% \author{M.~Laurenza}\affiliation{\instRomaTreINFN}\affiliation{\instRomaTreUNIV} % RomaTre
% \author{I.~S.~Lee}\affiliation{\instHanyang} % Hanyang
% \author{J.~K.~Lee}\affiliation{\instSeoul} % Seoul
  \author{S.~C.~Lee}\affiliation{\instKyungpook} % Kyungpook
% \author{D.~Levit}\affiliation{\instKEK} % KEK
  \author{P.~Lewis}\affiliation{\instBonn} % Bonn
% \author{C.~H.~Li}\affiliation{\instLNNU} % LNNU
% \author{J.~Li}\affiliation{\instKyungpook} % Kyungpook
  \author{L.~K.~Li}\affiliation{\instCincinnati} % Cincinnati
% \author{S.~X.~Li}\affiliation{\instFudan} % Fudan
  \author{Y.~Li}\affiliation{\instFudan} % Fudan
% \author{Y.~B.~Li}\affiliation{\instFudan} % Fudan
  \author{L.~Li~Gioi}\affiliation{\instMPP} % MPI
  \author{J.~Libby}\affiliation{\instIITMadras} % IITM
  \author{K.~Lieret}\affiliation{\instLMU} % LMU
  \author{Y.-R.~Lin}\affiliation{\instNTUTaiwan} % Taiwan
% \author{Z.~Liptak}\affiliation{\instHiroshima} % Hiroshima
  \author{D.~Liventsev}\affiliation{\instWayneState}\affiliation{\instKEK} % WayneState
  \author{T.~Luo}\affiliation{\instFudan} % Fudan
% \author{J.~MacNaughton}\affiliation{\instUOM} % NPC
% \author{A.~Martini}\affiliation{\instDESY} % DESY
  \author{M.~Masuda}\affiliation{\instEri}\affiliation{\instRCNP} % NPC
  \author{T.~Matsuda}\affiliation{\instUOM} % NPC
  \author{D.~Matvienko}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{S.~K.~Maurya}\affiliation{\instIITGuwahati} % IITG
  \author{F.~Meier}\affiliation{\instDuke} % Duke
  \author{M.~Merola}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % Napoli
  \author{F.~Metzner}\affiliation{\instBonn} % Bonn
  \author{K.~Miyabayashi}\affiliation{\instNaraWu}\affiliation{\instKEK} % Nara
% \author{H.~Miyake}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{H.~Miyata}\affiliation{\instNiigata} % Niigata
% \author{R.~Mizuk}\affiliation{\instHSE} % HSE
  \author{G.~B.~Mohanty}\affiliation{\instTata} % Tata
% \author{H.~K.~Moon}\affiliation{\instKoreaUnivKU} % Korea
% \author{T.~J.~Moon}\affiliation{\instSeoul} % Seoul
% \author{H.-G.~Moser}\affiliation{\instMPP} % MPI
% \author{M.~Mrvar}\affiliation{\instHEPHYVienna} % Vienna
% \author{T.~M\"uller}\affiliation{\instKarlsruhe} % Karlsruhe
  \author{R.~Mussa}\affiliation{\instTorinoINFN} % Torino
  \author{I.~Nakamura}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{K.~R.~Nakamura}\affiliation{\instKEK} % KEK
% \author{E.~Nakano}\affiliation{\instOsakaMetropolitan} % OsakaCity
  \author{T.~Nakano}\affiliation{\instRCNP} % NPC
  \author{M.~Nakao}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{H.~Nakayama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{H.~Nakazawa}\affiliation{\instNTUTaiwan} % Taiwan
% \author{D.~Narwal}\affiliation{\instIITGuwahati} % IITG
  \author{Z.~Natkaniec}\affiliation{\instKrakow} % Krakow
  \author{A.~Natochii}\affiliation{\instHawaii} % Hawaii
  \author{L.~Nayak}\affiliation{\instIITHyderabad} % IITH
  \author{M.~Nayak}\affiliation{\instTelAviv} % TelAviv
% \author{C.~Niebuhr}\affiliation{\instDESY} % DESY
% \author{M.~Niiyama}\affiliation{\instKSU} % NPC
  \author{N.~K.~Nisar}\affiliation{\instBNL} % BNL
  \author{S.~Nishida}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{K.~Nishimura}\affiliation{\instHawaii} % Hawaii
% \author{K.~Ogawa}\affiliation{\instNiigata} % Niigata
  \author{S.~Ogawa}\affiliation{\instToho} % Toho
% \author{S.~Okuno}\affiliation{\instKanagawa} % Kanagawa
% \author{S.~L.~Olsen}\affiliation{\instCAU} % CAU
  \author{H.~Ono}\affiliation{\instNDU}\affiliation{\instNiigata} % NihonDental
% \author{Y.~Onuki}\affiliation{\instUTokyo} % Tokyo
  \author{P.~Oskin}\affiliation{\instIJCLab} % IJCLab
% \author{H.~Ozaki}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
  \author{P.~Pakhlov}\affiliation{\instHSE} % HSE
  \author{G.~Pakhlova}\affiliation{\instHSE} % HSE
% \author{T.~Pang}\affiliation{\instPittsburgh} % Pittsburgh
  \author{S.~Pardi}\affiliation{\instNapoliINFN} % Napoli
  \author{H.~Park}\affiliation{\instKyungpook} % Kyungpook
  \author{J.~Park}\affiliation{\instYonsei} % Yonsei
% \author{S.-H.~Park}\affiliation{\instKEK} % KEK
% \author{A.~Passeri}\affiliation{\instRomaTreINFN} % RomaTre
  \author{S.~Patra}\affiliation{\instIISER} % IISERM
  \author{S.~Paul}\affiliation{\instTUM}\affiliation{\instMPP} % TUM
% \author{T.~K.~Pedlar}\affiliation{\instLuther} % Luther
  \author{R.~Pestotnik}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{F.~Pham}\affiliation{\instMelbourne} % Melbourne
  \author{L.~E.~Piilonen}\affiliation{\instVPI} % VPI
  \author{T.~Podobnik}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{V.~Popov}\affiliation{\instHSE} % HSE
% \author{S.~Prell}\affiliation{\instISU} % ISU
  \author{E.~Prencipe}\affiliation{\instGiessen} % Giessen
  \author{M.~T.~Prim}\affiliation{\instBonn} % Bonn
% \author{M.~V.~Purohit}\affiliation{\instOkinawa} % OIST
% \author{A.~Rabusov}\affiliation{\instTUM} % TUM
% \author{M.~Ritter}\affiliation{\instLMU} % LMU
% \author{M.~R\"{o}hrken}\affiliation{\instDESY} % DESY
  \author{A.~Rostomyan}\affiliation{\instDESY} % DESY
  \author{N.~Rout}\affiliation{\instIITMadras} % IITM
% \author{M.~Rozanska}\affiliation{\instKrakow} % Krakow
  \author{G.~Russo}\affiliation{\instNapoliUNIV} % Napoli
% \author{D.~Sahoo}\affiliation{\instISU} % ISU
% \author{Y.~Sakai}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{M.~Salehi}\affiliation{\instMalaya}\affiliation{\instLMU} % Malaya
  \author{S.~Sandilya}\affiliation{\instIITHyderabad} % IITH
% \author{A.~Sangal}\affiliation{\instCincinnati} % Cincinnati
  \author{L.~Santelj}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{T.~Sanuki}\affiliation{\instTohoku} % Tohoku
  \author{V.~Savinov}\affiliation{\instPittsburgh} % Pittsburgh
% \author{P.~Schmolz}\affiliation{\instLMU} % LMU
% \author{O.~Schneider}\affiliation{\instEPFL} % Lausanne
  \author{G.~Schnell}\affiliation{\instBilbao}\affiliation{\instIKERBASQUE} % Bilbao
  \author{J.~Schueler}\affiliation{\instHawaii} % Hawaii
  \author{C.~Schwanda}\affiliation{\instHEPHYVienna} % Vienna
% \author{A.~J.~Schwartz}\affiliation{\instCincinnati} % Cincinnati
% \author{B.~Schwenker}\affiliation{\instGoettingen} % Goettingen
% \author{R.~Seidl}\affiliation{\instRIKENBNL} % RIKEN
  \author{Y.~Seino}\affiliation{\instNiigata} % Niigata
  \author{K.~Senyo}\affiliation{\instYamagata} % Yamagata
% \author{O.~Seon}\affiliation{\instNagoya} % Nagoya
  \author{M.~E.~Sevior}\affiliation{\instMelbourne} % Melbourne
  \author{W.~Shan}\affiliation{\instHUNNU} % HUNNU
  \author{M.~Shapkin}\affiliation{\instIHEPRussia} % Protvino
  \author{C.~Sharma}\affiliation{\instMNITJaipur} % MNIT
% \author{V.~Shebalin}\affiliation{\instHawaii} % Hawaii
  \author{C.~P.~Shen}\affiliation{\instFudan} % Fudan
% \author{H.~Shibuya}\affiliation{\instToho} % Toho
  \author{J.-G.~Shiu}\affiliation{\instNTUTaiwan} % Taiwan
% \author{B.~Shwartz}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
% \author{A.~Sibidanov}\affiliation{\instHawaii} % Hawaii
  \author{F.~Simon}\affiliation{\instMPP} % MPI
% \author{J.~B.~Singh}\affiliation{\instPanjab}\affiliation{\instUPES} % Panjab
% \author{R.~Sinha}\affiliation{\instChennai} % IMSC
% \author{K.~Smith}\affiliation{\instMelbourne} % Melbourne
  \author{A.~Sokolov}\affiliation{\instIHEPRussia} % Protvino
% \author{Y.~Soloviev}\affiliation{\instDESY} % DESY
  \author{E.~Solovieva}\affiliation{\instBINP} % BINP
% \author{S.~Stani\v{c}}\affiliation{\instNovaGorica} % NovaGorica
  \author{M.~Stari\v{c}}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{Z.~S.~Stottler}\affiliation{\instVPI} % VPI
% \author{J.~F.~Strube}\affiliation{\instPNNL} % PNNL
% \author{J.~Stypula}\affiliation{\instKrakow} % Krakow
  \author{M.~Sumihama}\affiliation{\instGifu}\affiliation{\instRCNP} % NPC
% \author{K.~Sumisawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI}\affiliation{\instNaraWu} % KEK
  \author{T.~Sumiyoshi}\affiliation{\instTokyoMetropolitan} % TMU
  \author{W.~Sutcliffe}\affiliation{\instBonn} % Bonn
% \author{S.~Y.~Suzuki}\affiliation{\instKEK} % KEK
  \author{M.~Takizawa}\affiliation{\instSPU}\affiliation{\instJPARC}\affiliation{\instRIKENMSL} % NPC
  \author{U.~Tamponi}\affiliation{\instTorinoINFN} % Torino
% \author{S.~Tanaka}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{S.~S.~Tang}\affiliation{\instFudan} % Fudan
% \author{N.~Taniguchi}\affiliation{\instKEK} % KEK
% \author{Y.~Tao}\affiliation{\instFlorida} % Florida
% \author{G.~N.~Taylor}\affiliation{\instMelbourne} % Melbourne
  \author{F.~Tenchini}\affiliation{\instPisaINFN}\affiliation{\instPisaUNIV} % Pisa
% \author{Y.~Teramoto}\affiliation{\instOsakaMetropolitan} % OsakaCity
% \author{A.~Thampi}\affiliation{\instJuelich} % Juelich
% \author{R.~Tiwary}\affiliation{\instTata} % Tata
% \author{K.~Trabelsi}\affiliation{\instIJCLab} % IJCLab
% \author{T.~Tsuboyama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
  \author{M.~Uchida}\affiliation{\instTitech} % NPC
% \author{I.~Ueda}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
  \author{S.~Uehara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
  \author{T.~Uglov}\affiliation{\instHSE} % HSE
  \author{Y.~Unno}\affiliation{\instHanyang} % Hanyang
  \author{K.~Uno}\affiliation{\instNiigata} % Niigata
  \author{S.~Uno}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
  \author{P.~Urquijo}\affiliation{\instMelbourne} % Melbourne
% \author{Y.~Ushiroda}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
  \author{Y.~Usov}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{S.~E.~Vahsen}\affiliation{\instHawaii} % Hawaii
  \author{R.~van~Tonder}\affiliation{\instBonn} % Bonn
  \author{G.~Varner}\affiliation{\instHawaii} % Hawaii
% \author{K.~E.~Varvell}\affiliation{\instSydney} % Sydney
  \author{A.~Vinokurova}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
% \author{V.~Vorobyev}\affiliation{\instBINP} % BINP
  \author{A.~Vossen}\affiliation{\instDuke} % Duke
% \author{E.~Waheed}\affiliation{\instKEK} % KEK
% \author{B.~Wang}\affiliation{\instMPP} % MPI
% \author{C.~H.~Wang}\affiliation{\instNUUTaiwan} % NUU
  \author{D.~Wang}\affiliation{\instFlorida} % Florida
% \author{E.~Wang}\affiliation{\instPittsburgh} % Pittsburgh
  \author{M.-Z.~Wang}\affiliation{\instNTUTaiwan} % Taiwan
% \author{X.~L.~Wang}\affiliation{\instFudan} % Fudan
  \author{M.~Watanabe}\affiliation{\instNiigata} % Niigata
% \author{Y.~Watanabe}\affiliation{\instKanagawa} % Kanagawa
  \author{S.~Watanuki}\affiliation{\instYonsei} % Yonsei
% \author{S.~Wehle}\affiliation{\instDESY} % DESY
  \author{O.~Werbycka}\affiliation{\instTriesteINFN} % Trieste
% \author{E.~Widmann}\affiliation{\instSMI} % Vienna
% \author{J.~Wiechczynski}\affiliation{\instKrakow} % Krakow
  \author{E.~Won}\affiliation{\instKoreaUnivKU} % Korea
  \author{X.~Xu}\affiliation{\instSoochow} % Soochow
  \author{B.~D.~Yabsley}\affiliation{\instSydney} % Sydney
% \author{S.~Yamada}\affiliation{\instKEK} % KEK
% \author{H.~Yamamoto}\affiliation{\instTohoku} % Tohoku
  \author{W.~Yan}\affiliation{\instUSTC} % USTC
  \author{S.~B.~Yang}\affiliation{\instKoreaUnivKU} % Korea
% \author{H.~Ye}\affiliation{\instDESY} % DESY
  \author{J.~H.~Yin}\affiliation{\instKoreaUnivKU} % Korea
% \author{Y.~Yook}\affiliation{\instIHEPChina} % IHEP
  \author{C.~Z.~Yuan}\affiliation{\instIHEPChina} % IHEP
  \author{L.~Yuan}\affiliation{\instBeihang} % Beihang
% \author{Y.~Yusa}\affiliation{\instNiigata} % Niigata
% \author{Y.~Zhai}\affiliation{\instISU} % ISU
% \author{J.~Zhang}\affiliation{\instIHEPChina} % IHEP
  \author{Z.~P.~Zhang}\affiliation{\instUSTC} % USTC
  \author{V.~Zhilich}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{V.~Zhukova}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{V.~Zhulanov}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
\collaboration{The Belle Collaboration}

